Mini-Proceedings of ECT Workshop "Strangeness in Nuclei"

This workshop brought together international experts in the research area of strangeness in nuclei physics, working on theory as well as on experiments, to discuss the present status, to develop new methods of analysis and to have the opportunity for brainstorming towards future studies, going towards a deeper understanding of the hot topics in the low-energy QCD in the strangeness sector.

==> pochodzalla/pochodzalla.tex <==
%%%%
% ECT* mini-proceedings 2010 template
% v1.0, 2010/10/10
%%%%

%
% The paper should be one page long.
%%%%

%%
% Preamble part
% Do not modify it
%%
%\documentclass[12pt,a4paper]{report}
%\setlength{\textwidth}{160mm}
%\setlength{\textheight}{250mm}
%\setlength{\headheight}{10mm}
%\setlength{\oddsidemargin}{0mm}
%\setlength{\evensidemargin}{0mm}
%\setlength{\topmargin}{-20mm}
%\setlength{\parindent}{0mm}

%\usepackage{amsmath}
%\usepackage{graphicx}

%\newcommand{\titl}[1]{{\centering\Large\bf #1\par}\bigskip}
%\newcommand{\name}[1]{{\centering\rm\normalsize #1\par}\bigskip}
%\newcommand{\pres}[1]{\underline{#1}}
%\newcommand{\adr}[1]{{\it \normalsize #1\par}\medskip}
%\newenvironment{abstr}{\par\medskip\setlength{\parindent}{10mm} \normalsize \rm}{\par\bigskip}
%\frenchspacing

%%
% Document start
%%
%\begin{document}

%%
% Title
%%
\titl{Hypernuclei - recent experimental observations and future opportunities}

%%
% Authors
%%
\name{
%%
%%
% Author list continues here
%%
Josef Pochodzalla
}

%%
% Affiliations
%%
\adr{Johannes Gutenberg-Universit\"at Mainz,
Institute f\"ur Kernphysik, 55099 Mainz, Germany
}

%%
% The paper itself
%%
Today we are at the verge of a new impact from the experiments planned or already operative at various laboratories all over the world. The complementary of these different experimental approaches to hypernuclei provides a wide basis for a comprehensive understanding of strange hadrons in cold hadronic matter.
\begin{itemize}
\item
At J-PARC hypernuclei will be produced by intense meson beams. Indeed hypernuclear physics is the main topic in several day-one experiments. The experiments will focus on the $\gamma$-spectroscopy of single $\Lambda$-hypernuclei, $\Xi$-hypernuclei by the missing mass method and ground state decays of double hypernuclei in hybrid-emulsion experiments.

\item
The HYPHI experiment at GSI is searching for hypernuclei in peripheral heavy ion collisions at energies around 2AGeV. Final results of the first experiment are expected early 2011.

\item
The STAR collaboration has recently reported the first observation of hypernuclei and anti-hypernuclei in relativistic heavy ion collisions. Also the FOPI collaboration has presented first preliminary results on the search hypernuclei. These results and the ongoing search for hypernuclei by the ALICE experiment at LHC open a new window towards the transition from a quark-gluon system to the common world of hadrons and complex nuclei. Heavy ion experiments will provide precise information on the lifetime on single hypernuclei. 

\item
The experimental program at JLAB has been completed and at the moment the 12GeV upgrade is going on. Several light hypernuclei have been studied by electro-production so far. The analysis of the latest experiments performed in 2009 is ongoing and new results are expected soon. The experimental program at JLAB is not expected to continue before 2012. The future program will focus on precision pion spectroscopy and the excitation spectrum of medium heavy single hypernuclei.

\item
With the commissioning of the 1.6 GeV electron beam of MAMI-C the study of hypernuclei has become possible in Mainz. Thus the activity at JLAB will be complemented by experiments planned at MAMI. The key elements of the experimental program at MAMI are the measurement of the angle distribution of the hypernuclei close to zero degree by missing mass studies and the precision pion spectroscopy.

\item
PANDA at FAIR will study double hypernuclei by high resolution $\gamma$-spectroscopy. This experiment complements measurements of ground state masses of double hypernuclei in emulsions at J-PARC or in heavy ion reactions. 
\end{itemize}

Even though a number of new experimental techniques have been developed in the field of hypernuclear physics in the last decade, our knowledge is still limited to a small number of hypernuclei on or near the  $\beta$-stability line. However several activities which are ongoing or planned for the next decade will focus on different observables thus helping to overcome the present limitation.

\end{document}

